Designing Search Tasks for Archive Search

Longitudinal corpora like legal, corporate and newspaper archives are of immense value to a variety of users, and time as an important factor strongly influences their search behavior in these archives. While many systems have been developed to support users temporal information needs, questions remain over how users utilize these advances to satisfy their needs. Analyzing their search behavior will provide us with novel insights into search strategy, guide better interface and system design and highlight new problems for further research. In this paper we propose a set of search tasks, with varying complexity, that IIR researchers can utilize to study user search behavior in archives. We discuss how we created and refined these tasks as the result of a pilot study using a temporal search engine. We not only propose task descriptions but also pre and post-task evaluation mechanisms that can be employed for a large-scale study (crowdsourcing). Our initial findings show the viability of such tasks for investigating search behavior in archives.

==> chapters/results.tex <==
\section{Results and Discussion} % (fold)
\label{sec:results_and_discussion}

\begin{enumerate}
	\item pre-task - how did users perceive the task
	\item post-task - how did users like the task? interest? time? difficulty of questions (performance)
	\item post-task discussions and suggestions
	\item system usage patterns
	\item improved tasks
\end{enumerate}

% section results_and_discussion (end)
